Non-invasive probing of random local potential fluctuations in ZnCdSe/ZnSe quantum wells

Temperature dependence and recombination behavior of trapped charge carriers in ZnCdSe/ZnSe multiple quantum wells are investigated employing surface acoustic waves. These weakly perturb the carrier system, but remain highly sensitive even at small conductivities. Using this non-invasive probe we are able to detect persistent photoconductivity minutes after optical excitation. Measurement of exciting photon energies, the temperature dependence and ability to quench the conductivity with energies lower than the bandgap, support the notion of spatial separation of electrons and holes in the wells, due to random local potential fluctuations possibly induced by compositional fluctuations.

==> references.tex <==
@Article{Rotter_PRL,
  title = {Charge Conveyance and Nonlinear Acoustoelectric Phenomena for Intense Surface Acoustic Waves on a Semiconductor Quantum Well},
  author = {Rotter, M.  and Kalameitsev, A. V. and Govorov, A. O. and Ruile, W.  and Wixforth, A. },
  journal = {Phys. Rev. Lett.},
  volume = {82},
  number = {10},
  pages = {2171--2174},
  numpages = {3},
  year = {1999},
  month = {Mar},
  doi = {10.1103/PhysRevLett.82.2171},
  publisher = {American Physical Society}
}
@article{couto_PRL,
author = {O. D. D. {Couto Jr}. and F. Iikawa and J. Rudolph and R. Hey and P. V. Santos},
collaboration = {},
title = {Anisotropic Spin Transport in (110) GaAs Quantum Wells},
publisher = {APS},
year = {2007},
journal = {Physical Review Letters},
volume = {98},
number = {3},
eid = {036603},
numpages = {4},
pages = {036603},
url = {http://link.aps.org/abstract/PRL/v98/e036603},
doi = {10.1103/PhysRevLett.98.036603}
}
@article{boedefeld_PRB,
author = {C. B\"{o}defeld and J. Ebbecke and J. Toivonen and M. Sopanen and H. Lipsanen and A. Wixforth},
collaboration = {},
title = {Experimental investigation towards a periodically pumped single-photon source},
publisher = {APS},
year = {2006},
journal = {Physical Review B (Condensed Matter and Materials Physics)},
volume = {74},
number = {3},
eid = {035407},
numpages = {5},
pages = {035407},
keywords = {surface acoustic waves; electron-hole recombination; semiconductor quantum dots; semiconductor quantum wells; piezoelectricity; photoluminescence},
url = {http://link.aps.org/abstract/PRB/v74/e035407},
doi = {10.1103/PhysRevB.74.035407}
}
@article{gell_APL,
author = {J. R. Gell and M. B. Ward and R. J. Young and R. M. Stevenson and P. Atkinson and D. Anderson and G. A. C. Jones and D. A. Ritchie and A. J. Shields},
collaboration = {},
title = {Modulation of single quantum dot energy levels by a surface-acoustic-wave},
publisher = {AIP},
year = {2008},
journal = {Applied Physics Letters},
volume = {93},
number = {8},
eid = {081115},
numpages = {3},
pages = {081115},
keywords = {energy states; III-V semiconductors; indium compounds; semiconductor quantum dots; surface acoustic waves},
url = {http://link.aip.org/link/?APL/93/081115/1},
doi = {10.1063/1.2976135}
}
@article{couto_NatPhot,
author = {O. D. D. {Couto Jr}. and S. Lazic and F. Iikawa and J. A. H. Stotz and U. Jahn and R. Hey and P. V. Santos},
collaboration = {},
title = {Photon anti-bunching in acoustically pumped quantum dots},
year = {2009},
journal = {Nat. Photon.},
volume = {3},
number = {11},
pages = {645-648},
doi = {10.1038/nphoton.2009.191}
}


@article{Lang,
  title = {{Trapping characteristics and a donor-complex ($DX$) model for the persistent-photoconductivity trapping center in Te-doped $Al_xGa_{1-x}As$}},
  author = {Lang, D. V. and Logan, R. A. and Jaros, M. },
  journal = {Phys. Rev. B},
  volume = {19},
  number = {2},
  pages = {1015--1030},
  numpages = {15},
  year = {1979},
  month = {},
  doi = {10.1103/PhysRevB.19.1015},
  publisher = {American Physical Society}
}
@article{Chang,
author = {C. W. Chang and H. C. Yang and C. H. Chen and H. J. Chang and Y. F. Chen},
collaboration = {},
title = {Optoelectronic properties of ZnSe/ZnMgSSe multiple quantum wells},
publisher = {AIP},
year = {2001},
journal = {Journal of Applied Physics},
volume = {89},
number = {7},
pages = {3725-3729},
doi = {10.1063/1.1350416}
}
@Article{Firszt,
  title = {{Persistent photoconductivity and optically stimulated luminescence in $Zn_{0.8}Mg_{0.2}Se$ mixed crystals}},
  author = {Firszt,F. and Meczynska,H. and Legowski,S. and Zakrzewski,J. and Strzalkowski,K. and Wrobel,M.},
  journal = {physica status solidi (c)},
  volume = {1},
  number = {4},
  pages = {4},
  numpages = {},
  year = {2004},
  month = {},
  doi = {},
  publisher = {}
}
@Article{PhysRevB.44.13343,
  title = {{Charge storage and persistent photoconductivity in a $CdS0.5$$Se0.5$ semiconductor alloy}},
  author = {Dissanayake, A. S. and Huang, S. X. and Jiang, H. X. and Lin, J. Y.},
  journal = {Phys. Rev. B},
  volume = {44},
  number = {24},
  pages = {13343--13348},
  numpages = {5},
  year = {1991},
  month = {},
  doi = {10.1103/PhysRevB.44.13343},
  publisher = {American Physical Society}
}

}
@Article{Jiang2,
title = {{Persistent photoconductivity and related critical phenomena in $Zn0.3$$Cd0.7$Se}},
  author = {Jiang, H. X. and Lin, J. Y.},
  journal = {Phys. Rev. B},
  volume = {40},
  number = {14},
  pages = {10025--10028},
  numpages = {3},
  year = {1989},
  month = {},
  doi = {10.1103/PhysRevB.40.10025},
  publisher = {American Physical Society}
}
@Article{PhysRevLett.64.2547,
  title = {{Percolation transition of persistent photoconductivity in II-VI mixed crystals}},
  author = {Jiang, H. X. and Lin, J. Y.},
  journal = {Phys. Rev. Lett.},
  volume = {64},
  number = {21},
  pages = {2547--2550},
  numpages = {3},
  year = {1990},
  month = {},
  doi = {10.1103/PhysRevLett.64.2547},
  publisher = {American Physical Society}
}
@Article{Jiang1,
author = {H. X. Jiang and G. Brown and J. Y. Lin},
collaboration = {},
title = {{Persistent photoconductivity in II-VI and III-V semiconductor alloys and a novel infrared detector}},
publisher = {AIP},
year = {1991},
journal = {Journal of Applied Physics},
volume = {69},
number = {9},
pages = {6701-6703},
keywords = {PHOTOCONDUCTIVITY; SEMICONDUCTOR ALLOYS; ENERGY GAP; FLUCTUATIONS; ALUMINIUM ARSENIDES; GALLIUM ARSENIDES; ZINC SELENIDES; CADMIUM SELENIDES},
url = {},
doi = {10.1063/1.348889}
}
@Article{PhysRevB.45.4520,
  title = {{Band-tail states in a $Zn0.3$$Cd0.7$Se semiconductor alloy probed by persistent photoconductivity}},
  author = {Jiang, H. X. and Dissanayake, A.  and Lin, J. Y.},
  journal = {Phys. Rev. B},
  volume = {45},
  number = {8},
  pages = {4520--4523},
  numpages = {3},
  year = {1992},
  month = {},
  doi = {10.1103/PhysRevB.45.4520},
  publisher = {American Physical Society}
}
@Article{PhysRevB.41.5178,
  title = {{Relaxation of stored charge carriers in a $Zn0.3$$Cd0.7$Se mixed crystal}},
  author = {Lin, J. Y. and Jiang,H. X.},
  journal = {Phys. Rev. B},
  volume = {41},
  number = {8},
  pages = {5178--5187},
  numpages = {9},
  year = {1990},
  month = {},
  doi = {10.1103/PhysRevB.41.5178},
  publisher = {American Physical Society}
}
@article{fuhrmann,
author = {D. A. Fuhrmann and A. Wixforth and A. Curran and J. K. Morrod and K. A. Prior and R. J. Warburton and J. Ebbecke},
collaboration = {},
title = {Surface acoustic wave mediated exciton dissociation in a ZnCdSe/LiNbO[sub 3] hybrid},
publisher = {AIP},
year = {2009},
journal = {Applied Physics Letters},
volume = {94},
number = {19},
eid = {193505},
pages = {193505},
keywords = {acousto-optical effects; cadmium compounds; excitons; II-VI semiconductors; photoluminescence; piezoelectric materials; semiconductor epitaxial layers; semiconductor quantum wells; surface acoustic waves; zinc compounds},
doi = {10.1063/1.3136862}
}
@article{liftoff,
author = {A. Balocchi and A. Curran and T. C. M. Graham and C. Bradford and K. A. Prior and R. J. Warburton},
collaboration = {},
title = {Epitaxial liftoff of ZnSe-based heterostructures using a II-VI release layer},
publisher = {AIP},
year = {2005},
journal = {Applied Physics Letters},
volume = {86},
number = {1},
eid = {011915},
numpages = {},
pages = {011915},
url = {},
doi = {10.1063/1.1844595}
}
@Article{PhysRevB.40.7874,
  title = {{Surface acoustic waves on GaAs/$Alx$$Ga1-x$As heterostructures}},
  author = {Wixforth, A.  and Scriba, J.  and Wassermeier, M.  and Kotthaus, J. P. and Weimann, G.  and Schlapp, W. },
  journal = {Phys. Rev. B},
  volume = {40},
  number = {11},
  pages = {7874--7887},
  numpages = {13},
  year = {1989},
  month = {Oct},
  doi = {10.1103/PhysRevB.40.7874},
  publisher = {American Physical Society}
}
@Article{simon96,
  title = {Coupling of surface acoustic waves to a two-dimensional electron gas},
  author = {Simon, Steven H.},
  journal = {Phys. Rev. B},
  volume = {54},
  number = {19},
  pages = {13878--13884},
  numpages = {6},
  year = {1996},
  month = {},
  doi = {10.1103/PhysRevB.54.13878},
  publisher = {American Physical Society}
}
@Article{PhysRevB.57.R6850,
  title = {Exciton ionization in a quantum well studied by surface acoustic waves},
  author = {Rocke, C.  and Govorov, A. O. and Wixforth, A.  and B\"ohm, G.  and Weimann, G. },
  journal = {Phys. Rev. B},
  volume = {57},
  number = {12},
  pages = {R6850--R6853},
  numpages = {3},
  year = {1998},
  month = {},
  doi = {10.1103/PhysRevB.57.R6850},
  publisher = {American Physical Society}
}
@Article{PhysRevB.51.4699,
  title = {{Band offsets and exciton binding energies in Zn$_{1-x}$Cd$_{x}$Se-ZnSe quantum wells grown by metal-organic vapor-phase epitaxy}},
  author = {Liaci, F. and Bigenwald, P. and Briot, O. and Gil, B. and Briot, N. and Cloitre, T. Aulombard},
  journal = {Phys. Rev. B},
  volume = {51},
  number = {7},
  pages = {4699--4702},
  numpages = {3},
  year = {1995},
  month = {},
  doi = {10.1103/PhysRevB.51.4699},
  publisher = {American Physical Society}
}
@article{PhysRevB.79.155318,
author = {E. A. Zhukov and D. R. Yakovlev and M. Gerbracht and G. V. Mikhailov and G. Karczewski and T. Wojtowicz and J. Kossut and M. Bayer},
collaboration = {},
title = {Spin coherence of holes and electrons in undoped CdTe/(Cd,Mg)Te quantum wells},
publisher = {APS},
year = {2009},
journal = {Phys. Rev. B},
volume = {79},
number = {15},
eid = {155318},
pages = {155318},
doi = {10.1103/PhysRevB.79.155318}
}
@article{0957-4484-12-4-346,
  author={V V Travnikov and V H Kaibyshev and N V Lomasov and S I Nesterov and V I Skopina and E M Tanklevskaya and J Puls and M Rabe and F Henneberger},
  title={{Resonant exciton-phonon spectra in a ZnCdSe/ZnSe single quantum well}},
  journal={Nanotechnology},
  volume={12},
  number={4},
  pages={602-606},
  url={},
  year={2001},
}
@Article{Queisser,
  title = {Decay kinetics of persistent photoconductivity in semiconductors},
  author = {Queisser, H. J. and Theodorou, D. E.},
  journal = {Phys. Rev. B},
  volume = {33},
  number = {6},
  pages = {4027--4033},
  numpages = {6},
  year = {1986},
  month = {Mar},
  doi = {10.1103/PhysRevB.33.4027},
  publisher = {American Physical Society}
}
@Article{PhysRevB.40.7091,
  title = {Dynamics of continuous-time random walk, fractal time dispersion, and fractional exponential time relaxation},
  author = {Liu, Fu-sui  and Chao, Wen },
  journal = {Phys. Rev. B},
  volume = {40},
  number = {10},
  pages = {7091--7095},
  numpages = {4},
  year = {1989},
  month = {},
  doi = {10.1103/PhysRevB.40.7091},
  publisher = {American Physical Society}
}
@Article{Dissanayake,
  title = {{Kinetics of persistent photoconductivity in $Al_{0.3}Ga_{0.7}As$ and $Zn_{0.3}Cd_{0.7}Se$ semiconductor alloys}},
  author = {Dissanayake, A.  and Elahi, M.  and Jiang, H. X. and Lin, J. Y.},
  journal = {Phys. Rev. B},
  volume = {45},
  number = {24},
  pages = {13996--14004},
  numpages = {8},
  year = {1992},
  month = {},
  doi = {10.1103/PhysRevB.45.13996},
  publisher = {American Physical Society}
}
@Article{PhysRev.156.850,
  title = {Excitons and the Absorption Edge in ZnSe},
  author = {Hite, G. E. and Marple, D. T. F. and Aven, M.  and Segall, B. },
  journal = {Phys. Rev.},
  volume = {156},
  number = {3},
  pages = {850--859},
  numpages = {9},
  year = {1967},
  month = {Apr},
  doi = {10.1103/PhysRev.156.850},
  publisher = {American Physical Society}
}
@article{Scholl1994491,
title = "Persistent photoconductivity in CdTe-based II-VI-semiconductors",
journal = "Solid State Communications",
volume = "91",
number = "6",
pages = "491 - 495",
year = "1994",
doi = "DOI: 10.1016/0038-1098(94)90792-7",
author = "S. Scholl and J. Gersch{\"{u}}tz and H. Sch{\"{a}}fer and F. Fischer and A. Waag and G. Landwehr"
}
@article{Sheinkman76,
title = "Long-term relaxation and residual conductivity of semiconductors",
journal = "Sov. Phys. Semicond.",
volume = "10",
number = "128",
pages = "128",
year = "1976",
author = "Sheinkman, M.K. and Shik, A. Ya. and Poluprovodn., Fiz. Tekh."
}
@article{baskin:195325,
author = {I. Baskin and B. M. Ashkinadze and E. Cohen and L. N. Pfeiffer},
collaboration = {},
title = {Luminescence flashes induced by microwave radiation in undoped GaAs quantum wells},
publisher = {APS},
year = {2009},
journal = {Phys. Rev. B},
volume = {79},
number = {19},
eid = {195325},
pages = {195325},
}
@article{lomascolo:1145,
author = {M. Lomascolo and M. Di Dio and D. Greco and L. Calcagnile and R. Cingolani and L. Vanzetti and L. Sorba and A. Franciosi},
collaboration = {},
title = {Free versus localized exciton recombination in Zn[sub 1 - x]Cd[sub x]Se/ZnSe multiple quantum wells},
publisher = {AIP},
year = {1996},
journal = {Applied Physics Letters},
volume = {69},
number = {8},
pages = {1145-1147},
keywords = {QUANTUM WELLS; ZINC SELENIDES; CADMIUM SELENIDES; EXCITONS; LOCALIZED STATES; PHOTOLUMINESCENCE; TIME DEPENDENCE},
url = {http://link.aip.org/link/?APL/69/1145/1},
doi = {10.1063/1.117086}
}
@article{Runge95,
title = "Relaxation kinetics and photoluminescence lineshape of excitons in II-VI semiconductor quantum wells",
journal = "physica status solidi (b)",
volume = "188",
number = "",
pages = "547",
year = "1995",
author = "E. Runge and A. Sch{\"{u}}lzgen and F. Henneberger and R. Zimmermann"
}
@Article{PhysRevB.54.8728,
  title = {Electron-assisted exciton transfer and long-lived electrons and holes in GaAs/$Alx$$Ga1-x$As quantum wells},
  author = {Ashkinadze, B. M. and Tsidilkovski, E.  and Linder, E.  and Cohen, E.  and Ron, Arza  and Pfeiffer, L. N.},
  journal = {Phys. Rev. B},
  volume = {54},
  number = {12},
  pages = {8728--8736},
  numpages = {8},
  year = {1996},
  month = {Sep},
  doi = {10.1103/PhysRevB.54.8728},
  publisher = {American Physical Society}
}


